A Deep Learning Strategy for Vehicular Floating Content Management

Floating Content (FC) is a communication paradigm for the local dissemination of contextualized information through D2D connectivity, in a way which minimizes the use of resources while achieving some specified performance target. Existing approaches to FC dimensioning are based on unrealistic system assumptions that make them, highly inaccurate and overly conservative when applied in realistic settings. In this paper, we present a first step towards the development of a cognitive approach to efficient dynamic management of FC. We propose a deep learning strategy for FC dimensioning, which exploits a Convolutional Neural Network(CNN) to efficiently modulate over time the resources employed by FC in a QoS-aware manner. Numerical evaluations show that our approach achieves a maximum rejection rate of3%, and resource savings of 37.5% with respect to the benchmark strategy

==> Related_work.tex <==
\section{Related Work}
\label{related_w}
%The related work storyboard goes from the application on FC in VANETs to the Anchor Zone optimization for resource saving using analytical and learning approaches.       

A performance modeling of FC in vehicular environment was made in~\cite{itc29} where authors try to model it through a variant of random waypoint mobility model called District Model. In this work, the authors model, measure, and analyze the main performance of a circular AZ, in several vehicular scenarios (i.e., industrial, residential, and city center) of Luxembourg City. A previous attempt to model FC in urban setting was made in~\cite{fc_urban_env} and~\cite{fc_urban_areas}. In particular this latter, authors placed several AZs over the city of Helsinki, Finland. The aim was to measure the critical condition~\cite{floating}, in order to make the contents do not \textit{sink} (i.e., the minimum condition to make the content available within the AZ for the whole duration of the simulation).  

In the past few years, a particular focus, due to the emergent technologies and the increased need of communication resources, lays on the Anchor Zone optimization. A distributed and centralized approach to this end was presented in~\cite{ours2017mobiworld}. The aim of this work is to estimate nodes density in order to place an Anchor Zone in pressure situations. In particular, partitioning the map into a radial grid, each vehicle shares its estimation to the seeder node that is interested in placing the AZ. 
%A partitioned approach, placing a grid over a map, was presented in \cite{mobihoc}. In this paper, authors optimize the storage and the spread of the content aiming to the desired performance gave by the number of nodes with content entering in the so-called zone of interest. As previously mentioned, authors reduced the AZ costs by using a cell-based approach. 
A first try where the AZ shape is based on the traffic situation has been presented in~\cite{MONET2017}. In this work, authors adapt AZ shape and timing according to the traffic condition. On the one hand, they place one or more circular AZs in emergent location (e.g., car crash intersection). They reduce or remove the AZ based on the application goals.         

Given the massive growth of sensors and new tools to develop more accurate vehicular networks simulations~\cite{sommer2011}, new approaches (e.g., machine learning), which arise to process a huge amount of date, suit the open challenges in VANET. In particular, authors in~\cite{congestion_predict}, via deep learning techniques (Neural Network and Boltzmann Machine) predict the traffic congestion in each link of Ningbo city, China using data provided by taxi equipped with Global Position System devices. Whereas, in~\cite{cluster_density}, the work aims to estimate nodes density on a specific set of the highway by clustering nodes via V2V communication, and creating a density map via V2I communication. The same approach has been used in~\cite{traffic_prediction} for traffic prediction. The authors trained a machine to weight specific traffic features in order to predict traffic mobility over several links.   

In the above analytical works, nodes move according to an arbitrary mobility model such as random direction, or random waypoint. This can be a rough mobility modelization for real vehicular mobility cases. 
Moreover, the presented models have limitations due to unrealistic assumption. For instance, they are based on average values to design real dynamic scenarios.

In previous works, the granularity of AZ configuration is in terms of area cover by a circular, rectangular or grid shape. This approach involves a resource waste when part of the AZ lays over a no vehicular zone. Last but not least, only a few features such as nodes density, in the previous approaches are taking into account which again, arises a rough modelization.   

The aim of this work is to achieve the desired message availability spreading the content efficiently over a roadway. The granularity has been reduced to a road level, the outcomes are time-variant, and the performance is measured in terms of cost level (defined by the cost function), and method accuracy. Finally, by using a deep learning approach, no mobility assumptions are made. 


==> cognitive_approach.tex <==

\section{Formulation of the optimization problem}

(intro)\\


%%def of cost functions
In what follows we define a cost function, which is proportional to the amount of resources employed by a CFC scheme, in terms of user memory and of bandwidth.
The component which takes into account the total amount of user memory employed is indicated with $C^{m}_{l,t}$, and it is equal to the mean total  number of users with content, \textbf{and of the content size}.
$$
C^{m}_{l,t}=V^c_{l,t}L
$$
where $L$ is the content size in bits.

%\subsection{Problem Formulation}
\begin{equation}
\label{func:cost}
    %\textit{\textbf{C}}^{t}=C_{m}_{l,t}+C_{b}^{l,t}.  
\end{equation}


Besides the technology used, to coordinate the communication area, and to spread the content in it, the bigger AZ, the higher costs (e.g., bandwidth used). 
When a link is part of the AZ, it has a cost based on the number of vehicles in it $n_{l,t}$, number of vehicles in contact $\lambda$, transmission range $Tx$, and average contact time between vehicles $t_{\lambda}$. let $V_{l,t}=V^c_{l,t}+V^{nc}_{l,t}$. The function $g$ in the equation~\ref{func:g} can be defined as follows: 
\[
C_{loss}^{t}=\sum_{l}a_{l,t} V_{l,t}\frac{\lambda_{l,t} Tx}{\tau_{l,t}}.
\]
%where $A^{t}_i$ is the binary state of the $i-th$ link at time $t$.



In each time interval $t$, the constraint on success ratio can be written as
\be
\frac{\sum_{l\in\mathcal{L}'}\alpha_{l,t}V_{l,t}}{\sum_{l\in\mathcal{L}'}n_{l,t}} \geq S_{des}
\ee

Finally, the objective function to minimize is  defined by $C^{t}$ (i.e., equation~\ref{func:cost}). 
\begin{problem}
\label{prob:1}
Given the links features set of considered roadmap $P^t$, find the Anchor Zone configuration $A^{t}$ which achieves the performance target in the subset of roads selected by the application. 
\begin{equation}
\label{c}
  \minimize_{\mathcal{A}}\  k\sum_{l}a_{l,t}V_{l,t}\alpha_{l,t}+\sum_{l}a_{l,t} V_{l,t}\frac{\lambda_{l,t} Tx}{\tau_{l,t}},
\end{equation}
with $k\geq0$ as coefficient of the relative weight between the two cost components, and $a^{t}\geq S_{des}$ within the subset of links required by the application.
\end{problem}

==> leftovers.tex <==
\section{intro}

Existing approaches to FC dimensioning are based on a coarse partitioning of users, which results in over-dimensioning. 

They are based on stationary assumption wherein practical settings, this applies to contents which are relatively long-lived (a few hours, and in contexts in which mobility patterns and features do not vary significantly during the content lifetime). 


Otherwise, a conservative approach is required again, based on the worst mobility conditions (in terms of nodes density and contact rate) during the considered time interval. This brings to severely over-dimensioning of the AZ and to massively overestimating the required amount of resources for achieving a specific performance goal. 


The stationary analysis is entirely useless for very short-lived contents (e.g., less than one hour), as it does not account for the transient and the dynamics of content diffusion. The stationary analysis does not address the issue of optimal content seeding (i.e., where to start spreading the content). 

In limit cases, the content must be seeded very frequently, thus defeating the purpose of FC as a mean of offloading cellular infrastructure.


% Existing approaches are also based on the implicit assumption that mobility is not affected by information spreading. However, in most scenarios of interest, this is not the case. In a disaster scenario, for instance, floating the information about where rescue is needed, or where resources are available/unavailable, or where are hazards, clearly changes mobility patterns in ways that affect FC performance in return. Similar issues are found in swarms of drones for rescue operations, and even in pedestrian mobility, for messages about commercial sales, about flash events, about terrorist attacks, just to name a few (add citation). 

In these applications, how to  adequately engineer the FC paradigm without jeopardizing the communication resources available locally, achieving a target application performance while minimizing resource usage (in terms of bandwidth and/or memory, depending on the specific context), is an open issue which stands in the way of a practical deployment of the FC paradigm in such scenarios.

They rely on an implicit assumption of homogeneity in space of the underlying user density and of the mobility pattern, which brings to estimating the contribution of each node only as a function of its distance from the ZOI. 


\textbf{As a consequence, the dimensioning strategies resulting from these approaches are vastly inefficient in realistic, heterogeneous settings,} frequently including a large amount of nodes with little or no contribution to persistence and availability of floating content. 


% with  the  observation  that  in  the  5G  era  and  beyondopportunistic communications will make more and more senseas  provider  of  context-rich  information,  or  information  withonly   local   validity,   as   well   as   a   tool   for   offloading   theinfrastructure  of  localized  information  transfers



SYSTEM MODEL



The method can model event-based mobility (i.e., nodes reacting to content received). However, a study of the traffic evolution is out of the scope of this work.

an arbitrary area which includes other mobility than the vehicular one (e.g., pedestrian, drone). In this work, we consider vehicular mobility. 

In other words, the only communication between vehicles is via V2V (single-hop), whereas via vehicle-to-infrastructure communication (V2I), the vehicles are informed about the subset of links where they are enabled to receive and send the message. The approach can be easily extended to a multi-hop protocol or to a \textit{full} V2I communication.   




The model provides a subset of $\textit{\textbf{l}}$ where nodes within it, are enabled to receive, and opportunistically share the content. 

\begin{defn}[Anchor Zone]
Given $\textit{\textbf{l}}$, the Anchor Zone $\textbf{A}$ is the set $\mathcal{L}$ of links that allow the opportunistic replication and\/or storage. $\mathcal{L}$ is a subset of $\textit{\textbf{l}}$. 
\end{defn}


In other words, the only communication between vehicles is via V2V (single-hop), whereas via vehicle-to-infrastructure communication (V2I), the vehicles are informed about the subset of links where they are enabled to receive and send the message. The approach can be easily extended to a multi-hop protocol or to a \textit{full} V2I communication.   

Within the link enabled for the opportunistic communication, nodes exchange and/or store the message which contains the list of enabled links.

In the case of a single seeder (for instance, a warning about a road accident), the request to message broadcast is managed by the infrastructure (i.e., the node interested to spread the message send a request to the infrastructure, then the via V2I communication the message is broadcast).\\

%We define an Anchor Zone (AZ) as a subset $\mathcal{L}\subseteq\textit{\textbf{l}}$ of the road grid.
In each link, content storage and exchange are probabilistic.


A COGNITIVE APPROACH

(previous works achieved the highest performance using $60$ min interval time length~\cite{congestion_predict})



The availability ranged between 0 and 1, and can be constrained to be over the desired value $S_{des}$, in one or more roads
$$a_j\geq S_{des},$$ 
where the $j-th$ link has been selected by the application.  


$$
C_{loss}^{t}=\sum_{i=1}^{N}A^{t}_i\frac{\lambda^{t}_i(V^{t}_c+V^{t}_{nc})_iTx^{t}_i}{t^{t}_{\lambda_i}}.
$$

FORMULATION


In order to shape the communication area, we discretize the time into several intervals wherein we collect the required date to provide the configuration for the next interval. Once collected the date, these are grouped (i.e., averaged over interval time length). We refer to this grouping operation with the term \textit{aggregation level}. In this work, all intervals have the same length.  


% The AZ evolution for the entire simulation time $T$, considering $N$ links, can be described as follows:
% $$
% \textit{\textbf{A}}=
% \begin{bmatrix} 
% A_{1}^{t_1} & A_{1}^{t_2} & \dots & A_{1}^{T}\\ 
% A_{2}^{t_1} & A_{2}^{t_2} & \dots & A_{2}^{T}\\
% \vdots  & \vdots  & \ddots & \vdots\\
% A_{N}^{t_1} & A_{N}^{t_2} & \dots & A_{N}^{T}\\
% \end{bmatrix}   
% $$
% where $A_{n}^{t}$ is the couple of probabilities for both exchange and storage the content within the link $n$ at time $t$. For instance, if $A_{n}^{t}=(0.7,0.6)$ it means that in the road $n$ vehicles can exchange the message with a probability $0.7$, and keep the content with a probability $0.6$. With $A^{t}$ or simply $A$, we refer to a column in $\textit{\textbf{A}}$ matrix which denotes the Anchor Zone configuration at time $t$ (i.e., the communication area at time $t$).

To efficiently shape the communication area, we need to learn the relation between the road and its features. 

If with $P^{t}$ we indicate the features set of all links at time $t$, the application cost $C^{t}_{app}$ and the transmission cost $C^t_{loss}$ are function of $A^tP^t$. 
Analytically,
\begin{equation}
\label{func:g}
C^{t}_{app}=g(A^{t}_{1}P^{t}_{1},A^{t}_{2}P^{t}_{2},\dots,A^{t}_NP^{t}_N)
\end{equation}
\begin{equation}
\label{func:h}
C^t_{loss}=h(A^{t}_{1}P^{t}_{1},A^{t}_{2}P^{t}_{2},\dots,A^{t}_NP^{t}_N)\end{equation} 
with functions $g,h:\mathbb{R}^{N_x p}\rightarrow\mathbb{R}$, and $p$ as the link feature set size.


As previously mentioned, we are aiming to save resources achieving the performance target defined by the application. 
Therefore, the  Anchor Zone configuration at time $t$ ($A^t$), has a cost $C^t_{loss}$ given by the resources used, and a related application performance cost $C^{t}_{app}$ to achieve the desired target. 

The evolution of both costs $C_{app}$ and $C_{loss}$ can be express as follows: 
$$
\textit{\textbf{C}}=
\begin{bmatrix} 
C_{app}^{t_1} & C_{app}^{t_2} & \dots & C_{app}^{T}\\ 
C_{loss}^{t_1} & C_{loss}^{t_2} & \dots & C_{loss}^{T}\\
\end{bmatrix}   
$$
which at time $t$: 



==> miaooo.tex <==
 CNN architecture shown in Table~\ref{tab:cnn_arc} columns \textit{Shape} and \textit{Parameters numbers} refer to the scenario studied in the Numerical Evaluation section.
 
 For each of these strategies, we considered a rate of active links which goes from $5\%$ up to $100\%$, as a .

==> misc-old/intro.tex <==
\section{Introduction}

%%%%%% intro
Traffic data network is drastically increasing due to the high demands for multimedia services such as video-streaming, web-browsing and file-downloading. According to the main forecast reports such as Cisco and Ericsson (add citation), global mobile traffic is estimated to 5-times growth over 2017. In order to guarantee users' quality of service or experience (QoS/QoE) new offloading techniques are required. 
%%%%%%% types of cellular network



New offloading techniques to cope with the explosive growth in mobile traffic volumes, %and for the use cases as well as quality of service (QoS), 
are a fundamental component of the next generation radio access network (5G). %In vehicular ad-hoc networks (VANETs), 
Part of the cellular traffic volume can be offloaded to vehicular-to-vehicular communication (V2V), leaving to the infrastructure the task of managing and coordinating the communication.
In this context, of special interest are communication paradigms such as Floating Content (FC), an opportunistic communication scheme for the local dissemination of information \cite{floating}.  %\gr{small intro of FC. Done!}.

FC as an infrastructure-less communication model, enables probabilistic contents storing in geographically constrained locations - denoted as \textit{Anchor Zone} (AZ) - and over a limited amount of time based on the application requirements.  
 
Since FC has been introduced, studies have focused mainly on its modeling, try to adjust it into several scenarios from the Internet of Things (IoT)~\cite{office} to the Vehicular Ad-hoc Network (VANET)~\cite{itc29}. FC is based on the AZ area, where the opportunistic-content-exchange between nodes takes place (e.g., pedestrians, vehicles or hybrid communication) making the content "float" without infrastructure needs. Only recently in~\cite{ours2017mobiworld}, a particular focus has fallen on Anchor Zone dimensioning. %%%%The gain respect to the other works
% However, in both paths, FC modeling and AZ reshaping, previous studies did not take into account the following main features: 
% \begin{itemize}
%   \item nodes mobility update on content received (i.e., event-based mobility),
%   \item anchor zone granularity in terms of road-grid which reduces the area not interest to the communication,
%   \item and, most notably, the high dynamic of nodes mobility which requires a time-based approach. 
% \end{itemize}
% This work adds to the FC state-of-the-art the above keys points. 
Existing approaches for FC dimensioning (e.g., \cite{office}, \cite{itc29}, and \cite{ours2017mobiworld}) present the following issues:
\begin{itemize}
\item They are based on a coarse partitioning of users, which results in over-dimensioning.
\item They are based on stationary assumption. In practical settings, this applies to contents which are relatively long-lived (a few hours, and in contexts in which mobility patterns and features do not vary significantly during the content lifetime). Otherwise, a conservative approach is required again, based on the worst mobility conditions (in terms of nodes density and contact rate) during the considered time interval. This brings to severely over-dimensioning of the AZ and to heavily overestimating the required amount of resources for achieving a specific performance goal.
\item The stationary analysis is completely useless for very short-lived contents (e.g., less than one hour), as it does not account for the transient and the dynamics of content diffusion.  
\item The stationary analysis does not address the issue of optimal content seeding (i.e., where to start spreading the content). In limit cases, the content must be seeded very frequently, thus defeating the purpose of FC as a mean of offloading cellular infrastructure.
\item Existing approaches are also based on the implicit assumption that mobility is not affected by information spreading. However, in most scenarios of interest, this is not the case. In a disaster scenario, for instance, floating the information about where rescue is needed, or where resources are available/unavailable, or where are hazards, clearly changes mobility patterns in ways that affect FC performance in return. Similar issues are found in swarms of drones for rescue operations, and even in pedestrian mobility, for messages about commercial sales, about flash events, about terrorist attacks, just to name a few. In these applications, how to  adequately engineer the FC paradigm without jeopardizing the communication resources available locally, achieving a target application performance while minimizing resource usage (in terms of bandwidth and/or memory, depending on the specific context), is an open issue which stands in the way of a practical deployment of the FC paradigm in such scenarios.
\end{itemize}

%%%Finally what we do!!!
%This study attempts to extend machine learning theory into floating content paradigm to tackle the traffic congestion issue.  
In this work, a machine learning (ML) approach has been used to adapt in real time FC parameters, in a way which achieves the target performance while minimizing the overall cost (modeled through a given cost function) during the whole simulation period. The model does not require any stationary assumption or any geographical roadway-map information. Moreover, we believe that the massive data volume, diversity features selection, and the tremendous number of dependencies, can be analyzed only via an ML-based approach.
Therefore, a Convolutional Neural Network (CNN), over more ML techniques, has been used to predict the AZ configuration achieving an accuracy of $89.7\%$ within a confidence rate of $98\%$. The CNN algorithm by the AZ configuration provides the optimal seeding strategy as well. Moreover, even if is out of the scope of this work, the method can be performed within an event-based mobility scenario. 
Finally, the predicted AZ configurations are more efficient than analytical model configurations in the state-of-the-art. 

Section~\ref{system_m} provides the system model and measurements, followed by Section~\ref{prob_f} which shows the notation used and the problem formulation. CNN structure is shown in Section~\ref{alg} whereas Section~\ref{N-e} presents the numerical evaluations. Finally, in Section~\ref{related_w} we provide the related work, whereas, Section~\ref{concl} concludes this paper.   


==> misc-old/intro_old.tex <==
\section{Introduction}

%%%%%% intro
New offloading techniques to cope with the explosive growth in mobile traffic volumes, %and for the use cases as well as quality of service (QoS), 
are a fundamental component of the next generation radio access network (5G). %In vehicular ad-hoc networks (VANETs), 
Part of the cellular traffic volume can be offloaded to vehicular-to-vehicular communications (V2V), leaving to the infrastructure the task of managing and coordinating the communication.
In this context, of special interest are communication paradigms such as Floating Content (FC), an opportunistic communication scheme for the local dissemination of information \cite{floating}.  %\gr{small intro of FC. Done!}.

 FC beeing an infrastructure-less communication model, enables probabilistic contents storing in geographically constrained locations - denoted as \textit{Anchor Zones} (AZ) - and over a limited amount of time (i.e., application-based).
 
Since FC has been introduced, studies have focused mainly on its modeling, try to adjust it into a variant of scenarios from the Internet of Things (IoT)~\cite{office} to the Vehicular Ad-hoc Network (VANET)~\cite{itc29}. In particular, FC is based on the AZ area, where the opportunistic content exchange between nodes takes place (e.g., pedestrians, vehicles or hybrid communication) making the content "floats" without infrastructure needs. Only recently in~\cite{ours2017mobiworld}, a particular focus has fallen on Anchor Zone dimensioning. %%%%The gain respect to the other works
% However, in both paths, FC modeling and AZ reshaping, previous studies did not take into account the following main features: 
% \begin{itemize}
%   \item nodes mobility update on content received (i.e., event-based mobility),
%   \item anchor zone granularity in terms of road-grid which reduces the area not interest to the communication,
%   \item and, most notably, the high dynamic of nodes mobility which requires a time-based approach. 
% \end{itemize}
% This work adds to the FC state-of-the-art the above keys points. 
Existing approaches for FC dimensioning present the following issues:
\begin{itemize}
\item They are based on a coarse partitioning of users, which results in over dimensioning;
\item They are based on stationary assumption. In practical settings this applies to contents which are relatively long lived (a few hours, and in contexts in which mobility patterns and features do not vary significantly during content lifetime. Otherwise, a conservative approach is required again, based on the worst mobility conditions (in terms of node densities and contact rate) during the considered time interval. And this brings to severely overdimensioning of the AZ and to heavily overestimating the required amount of resources for achieving a specific performance goal.
\item The stationary analysis is completely useless for very short lived contents (less than one hour), as it does not accounts for the transient and the dynamics of content diffusion.  
\item The stationary analysis does not address the issue of optimal content seeding. In limit cases, the content must be seeded very frequently, thus defeating the purpose of FC as a mean of offloading cellular infrastructure.
\item Existing approaches are also based on the implicit assumption that mobility is not affected by information spreading. However, in most scenarios of interest, this is not the case. In a disaster scenario, for instance, floating the information about where rescue is needed, or where resources are available/unavailable, or where are hazards, clearly changes mobility patterns in ways that affect FC performance in return. Similar issues are found in swarms of drones for find and rescue operations, and even in pedestrian mobility, for messages about commercial sales, about flash events, about terrorist attacks, just to name a few. In these applications, how to  adequately engineer the FC paradigm without jeopardizing the communication resources available locally, achieving a target application performance while minimizing resource usage (in terms of bandwidth and/or memory, depending on the specific context), is an open issue which stands in the way of a practical deployment of the FC paradigm in such scenarios.
\end{itemize}
%
%%%Finally what we do!!!
%This study attempts to extend machine learning theory into floating content paradigm to tackle the traffic congestion issue.  
In this work, a machine learning (ML) approach has been used to adapt in real time FC parameters, in a way which achieves the target performance while minimizing the overall cost (modeled through a given cost function) during the whole duration of the congestion period. The model does not require any stationary assumption nor any geographical roadway-map information. Moreover, we believe that a massive data volume, variety features selection, and a tremendous number of dependency, can be analyzed only via an ML-based approach.
Therefore, a Convolutional Neural Network (CNN) over more ML techniques, has been used to predict the AZ configuration achieving an accuracy of $89.7\%$ within a confidence rate of $95\%$. Moreover, the predicted AZ configurations provide minor costs over the state-of-the-art results.   

Section~\ref{system_m} provides the system model assumption and measurements followed by Section~\ref{prob_f} which shows the notation used and the faced problem. CNN structure is shown in Section~\ref{alg} whereas Section~\ref{N-e} performs the numerical evaluations. Finally, in Section~\ref{related_w} we provide the related work, whereas, Section~\ref{concl} concludes this work.   


==> misc-old/system_model.tex <==
\section{System model}
We place a grip over a map where nodes move according to an arbitrary mobility mode. We assume to have the contact heat map for each cell (i.e., we know the coordination and the time when two or more nodes are in range according to the Gilbert’s model). For each cell...

==> old.tex <==
\section{Problem Statement 2: circular AZ resizing subject to success ratio target (old try)}
\textbf{General goal:}  
The problem to save resources (such as bandwidth, spectrum, memory storage, energy) by using Floating Content approach in vehicular context. 

\textbf{State of the art:}
Previous works on FC focused mainly on the study of the probability of content floating, availability, and success probability performances. 


\textbf{Specific goal:}
In spite of FC constraints geographically information-spreading,
\textit{how to optimize resources used by FC over AZ size and shape is still an open challenge}. 

Our primary goal is to save resources reserving a certain level of FC performance. This can be done in several ways. For instance, without using an opportunistic replication but selecting which node is allowed to receive the content and which is not. Another approach, to efficiently save resources, is to choose a different shape than circular for the AZ (e.g., rectangular for a highway).   

In this work, we face the problem of circular anchor zone resizing (i.e., select the best radius) in order to reduce the amount of nodes involved in the communication preserving the target performances.  

\textbf{System model:}
We consider a $\mathbb{R}^2$ space where nodes move according to an arbitrary distribution. Assuming a stationary state, we suppose to know the mean moving time $T_m$, respectively the mean static time $T_s$ of the nodes.
We assume that nodes transmission range $r$ is the same for all the nodes (which can be extended for an arbitrary distribution). By contact, we refer to Gilbert's model. It means that a contact event happens when the distance between two nodes is less than $r$. We place a circular AZ with radius $R$, and we indicate the mean node sojourn time within AZ  as $T_{soj}$, the mean speed nodes as $v$, and the mean arrival rate as $\lambda$. 


\textbf{Approach:}
We consider a basic setting of FC with a circular AZ placed in XY. Following, \textit{we estimate, through a machine learning approach, the minimum AZ radius subject to some performance parameters} (e.g., target success rate) and applications requirements (e.g., a minimum, a maximum or both AZ size).   

\textbf{Main differences from our previous work:}
 Our earlier work, it is model based. This means that each gear, in the general process %shown in Fig.~\ref{fig:machine}
 , is given by the model took into account. However, in this work, we tackle the same issue without considering any model, and we want that the data give these gears. This is a machine learning problem.
 Moreover, in this work, we do not consider the homogeneity node density within AZ as in the previous work (i.e., we do not assume that nodes are uniformed distributed within AZ).
% \begin{figure}[h]
%  \begin{center}
%     \includegraphics[width=\columnwidth]{Presentation1.pdf}
% \caption{General process}
% \label{fig:machine}
% \end{center}
% \end{figure}

\textbf{Features:}
As a first attempt, we take into account $T_s$, $T_m$, $T_{soj}$, $\lambda$, $v$, $r$, $R$ as features. Moreover, we must consider application requirement such as minimum and maximum radius (resp. $R_{min}$, $R_{max}$). 


\textbf{Output:}
The output of our machine learning algorithm is $R$.
%which respect the application performances such as $R_{min}$, $R_{max}$, and target success probability $P_{succ}$


\textbf{Training set:}
The training set contains all the features previous mentioned. The larger, the better particularly using a deep learning technique. The training set vector values must be normalized in order to avoid local optimization. The \textit{p-norm} is the most suitable normalization for the types of features chosen. 


\textbf{Which learning is it:} 
The output of the machine is the value of $R \in \mathbb{R}$ which respect all the requirements. This is regression problem. 

\textbf{Machine learning technique}
Deep Boltzmann machine \textbf{(explain why or other option)}

\gr{Fundamental issue: Mobihoc again solves optimally this problem, and by not limiting shapes to circular, does better on average, than whatever you propose. there's no fundamental reason why you should limit AZ shape to circular.}




==> statement.tex <==
\section{Problem Statement 1: Floating Content Strategy to Avoid Traffic Congestion Using Machine Learning Theory}

%\gr{try again to define the problem you want to solve, in a way that does not leave room for interpretation.}


The fundamental idea is to use Floating Content to solve traffic congestion problem, by \textit{spreading the information concerning this issue, in the areas nearby the congestion zone}. We want to place the anchor zone (AZ), to inform other vehicles \textbf{to avoid} traffic hot-spots (congestion areas). To this end,  we need first to detect high-density vehicular areas then place the AZ in the most efficient zone (i.e., efficient in terms of resource usage and success ratio within the interest area).\\
%\gr{Unintelligible. what is the problem? what do you want to achieve?}\\

The problem can be split into two sub-problems: the \textit{traffic congestion detection (TCD)}, \textit{identification of the congestion zone}, that can be reused from the state of the art or by an ad-hoc algorithm,
%\gr{define accurately TC, and define TCD. What do you want to do? detect congestion? avoid congestion??}\\
and \textit{anchor zone positioning} in order to prevent other vehicles to enter the congestion area, where the core of our work is.\\

Placing a grid over a given map, where nodes move according to an arbitrary mobility model, we define $C_{congest}$ as the set of cells congested. $C_{congest}$ for instance, can be evaluated considering a mean speed threshold, below which the cells are congested. $C_{interest}$ is the set of cells interested to spread and store the content in order to inform all the nodes close to $C_{congest}$. Summarizing, $C_{congest}$ defines the congestion zones whereas, $C_{interest}$ defines the Anchor Zone. Finally, the aim of this work is to evaluate the minimum $C_{interest}$, given $C_{congest}$, and a success ratio target.   


As the first attempt, we assume that we do not change nodes mobility but only report the congestion issue. 





To face this issue, we use machine learning theory. So, without any analytical model to describe our scenario, we train the machine to extract the best area to place the AZ. Therefore, placing a grid on the whole region, via machine learning method we select which cells activate for content exchanging and storage. 

The training set features, machine learning techniques, and optimization part are still a work in progress. State of the art must be explored in deep. \\

\gr{No different than Mobihoc paper, which solves this issue optimally.}


















==> statement3.tex <==
\section{Problem Statement 3: A Floating Content Distributed Seeding Approach for Car Crash Situation}
To the best of our knowledge, previous works on floating content did not focus on seeding strategies. This open challenge, involve effects such as content sink and information spreading transitory which strongly influence any model performance outcomes.      
We consider a city map, where nodes move according an arbitrary distribution. At a specific time, a car crash occurred. A percentage of vehicles, surrounded the emergency zone have been selected as seeders (nodes that generate the message). The aim of this work, is to obtain the minimum seeding area subject to a success probability target measured over the board of a fixed AZ. Figure \ref{fig:seed_area} shows the crash location (in red), the seeding area (in blue), and the Anchor Zone (in black). 
\begin{figure}[h]
 \begin{center}
    \includegraphics[width=0.5\columnwidth]{seed_area.PNG}
\caption{Anchor Zone, seeding area and crash location}
\label{fig:seed_area}
\end{center}
\end{figure}

\gr{Seeding optimization is a relatively marginal issue}




==> statement_4.tex <==
\section{Problem formulation 4}

Considering stationary conditions is ok only for relatively stable settings and long lived contents.
In settings where mobility changes rapidly, and for short lived contents (1H or less), modeling of spatio temporal content evolution
becomes important.\\
You can start from Karlsson paper, and apply mobihoc approach.
The optimization problem now is an optimization over temporal sequences of choices for the replication and storage variables. 
Solving this optimally is the challenge. And you do not need necessarily machine learning for this.

\section{Problem 5}

Find a problem for which ML and the alike are a very good choice.

\section{Problem 6}
Same as problem 4, with the additional complication of having traffic react and change patterns as a consequence of information diffusion. You need a reasonable model for how traffic reacts to information, and solve 4 OPTIMALLY.
This is the coolest problem of all, so far.



==> todo.tex <==
\section{ToDo}
\begin{itemize}
    \item Problem Formulation    \begin{itemize}
        \item Street not ON/OFF but with probability of exchange or to store (real number not binary)
    \end{itemize}
    \item Algorithm
    \begin{itemize}
        \item Explore different values of availability target
    \end{itemize}
    \item Numerical Evaluation
    \begin{itemize}
        \item Other real mobility
        \item Different aggregation level
        \item Explore the best Tx radius choice
    \end{itemize}
    \item cambia notazione secondo le indicazioni fornite.
    \item \textbf{which criteria to follow in determining links? Da spiegare da qualche parte.}
    \item di' che e' estendibile a non grid
    \item \textbf{(le auto appaiono? scompaiono?)} cosa succede quando si fermano?
    \item discuti durata intervalli e numero
    
    
    
\end{itemize}
